Robust Resilient Signal Reconstruction under Adversarial Attacks

We consider the problem of signal reconstruction for a system under sparse signal corruption by a malicious agent. The reconstruction problem follows the standard error coding problem that has been studied extensively in the literature. We include a new challenge of robust estimation of the attack support. The problem is then cast as a constrained optimization problem merging promising techniques in the area of deep learning and estimation theory. A pruning algorithm is developed to reduce the ``false positive" uncertainty of data-driven attack localization results, thereby improving the probability of correct signal reconstruction. Sufficient conditions for the correct reconstruction and the associated reconstruction error bounds are obtained for both exact and inexact attack support estimation. Moreover, a simulation of a water distribution system is presented to validate the proposed techniques.

==> sections/5-simulation.tex <==

\subsection{Data-Driven system}
Suppose, instead of the linear model in \eqref{eqn:global_LS}, one only has available the synchronous data tuple $\left\{\bs{\sigma}_i,\mathbf{y}_i\right\}$, $i=1,\hdots N_d$, where $\mathbf{y}_i\in\mathbb{R}^m$ are measurements collected from the process of interest and $\bs{\sigma}_i\in\mathbb{R}^{n_\sigma}$ are associated vectors of exogenous monitoring variables\footnote{These are supporting source of measurement which are assumed to be secure. Examples of such include; ambient conditions, external vibration measurements, thermal images, network login information, etc}. Let $f(.;\mathbf{p}):\mathbb{R}^{n_\sigma}\mapsto\mathbb{R}^m$ be a parametrized nonlinear mapping with parameter $\mathbf{p}$ selected to minimize the empirical loss function:
\begin{align}
J(\mathbf{p}) = \frac{1}{N_d}\sum\limits_{i=1}^{N_d}{\norm{\mathbf{y}_i-f(\bs{\sigma}_i;\mathbf{p})}^2}.
\end{align}
If $N_d$  is big enough, the residual $\left\{\mathbf{y}_i-f(\bs{\sigma}_i;\mathbf{p}^*)\right\}$ can be assumed to be unbiased. Thus, a linear model of the uncertainty can be obtained by a subspace reduction on the residual data. This can be obtained for instance by performing a principal component analysis (PCA) dimensionality reduction on the error covariance matrix
\begin{align*}
E = \frac{1}{N_d}\sum\limits_{i=1}^{N_d}{\left(\mathbf{y}_i-f(\bs{\sigma}_i;\mathbf{p}^*)\right)\left(\mathbf{y}_i-f(\bs{\sigma}_i;\mathbf{p}^*)\right)^\top}.
\end{align*}
Let $\Phi\in\mathbb{R}^{m\times n}, n<m$ be a matrix whose columns correspond to the first principal vectors of $E$. Then the data-driven linear model of the process to be used for resilient reconstruction is given by
\begin{align}
\mathbf{y} = f(\bs{\sigma};\mathbf{p}^*) + \Phi\mathbf{x} + \bs{\nu} + \mathbf{e},
\end{align}
with the model error bound $\norm{\bs{\nu}}\le\mathcal{O}(s_{n+1})$, where $s_k$ is the $k$th singular value of $E$. 

Thus, given $T=\textsf{supp}(\mathbf{e})$ with $\abs{T}>=n$ and $T^c\triangleq \{1,\hdots,m\}\backslash T$, the reconstruction is obtained as follows:
\begin{equation}
\begin{aligned}
\hat{\mathbf{x}} &= \argmin\limits_{\mathbf{x}\in\mathcal{X}}{\norm{\mathbf{y}_\mathcal{T}-{f(\bs{\sigma};\mathbf{p}^*)}_T-\Phi_{\mathcal{T}}\mathbf{x}}^2}\\
\hat{\mathbf{y}}_{\mathcal{T}} &=\mathbf{y}_\mathcal{T}\\
\hat{\mathbf{y}}_{\mathcal{T}^c} &= {f(\bs{\sigma};\mathbf{p}^*)}_{\mathcal{T}^c}-\Phi_{\mathcal{T}^c}\hat{\mathbf{x}}
\end{aligned}
\end{equation}
with the reconstruction error given by Corollary~\ref{cor:constrained_LS}.


\subsection{Linear Dynamical System}\label{Case}

Consider the discrete LTI system
\begin{align}
\mathbf{x}_{k+1}&=A\mathbf{x}_k\\
\mathbf{y}_k& = C\mathbf{x}_k + \mathbf{e}_k,
\end{align}
\noindent where $\mathbf{x}_k\in\mathbb{R}^n$ represents the state of the system at time $k\in\mathbb{N}$, $\mathbf{y}_k\in\mathbb{R}^m$ is the output of the monitoring nodes at time $k$ and $\mathbf{e}_k\in\mathbb{R}^m$ denote the attack signals injected by malicious agents at the monitoring nodes. Let $\mathcal{K} \subset \{1,2,\hdots,m\}$ denote the set of attacked nodes, then for all $k$, $\abs{\supp(\mathbf{e}_k)}\subset\mathcal{K}$. The resilient estimation problem is then defined as reconstructing the initial state $\mathbf{x}_0$ from corrupt measurement $\left\{\mathbf{y}_k\right\}_{k=0}^T, T\in\mathbb{N}$. We look at two scenarios from literature: $\mathcal{K}$ is time-invariant \cite{pasqualetti2013attack, fawzi2014secure} and $\mathcal{K}$ is time-varying\cite{hu2016secure}.
\subsubsection{Secure estimation for Fixed Attacked Nodes\cite{fawzi2014secure}}
Assuming that the set $\mathcal{K}$ of attacked nodes is time-invariant:
\begin{definition}\label{def:K_invariant}
$q$ errors are correctable after $T$ steps by the decoder $\mathcal{D}:\left(\mathbb{R}^m\right)^T\mapsto\mathbb{R}^n$ if for any $\mathbf{x}_0\in\mathbb{R}^n$, any $\mathcal{K}\subset\left\{1,2,\hdots,m\right\}$ with $\abs{\mathcal{K}}\le q$, and any sequence of vectors $\mathbf{e}_0,\hdots,\mathbf{e}_{T-1}\in\mathbf{R}^m$ such that $\supp(\mathbf{e}_k)\subset\mathcal{K}$, we have $\mathcal{D}(\mathbf{y}_0,\hdots,\mathbf{y}_{T-1})=\mathbf{x}_0$, where $\mathbf{y}_k = CA^k\mathbf{x}_0 + \mathbf{e}_k$ for $k=0,1,\hdots,T-1$.
\end{definition}

\begin{proposition}
Let $T \in \mathbb{N}  \backslash \{ 0\}$. The following are equivalent:\\
(i) There is a decoder that can correct $q$ errors after $T$ steps;\\
(ii) For all $\mathbf{z}\in \mathbb{R}^n \backslash \{0\}$, $\lvert \supp(C\mathbf{z}) \cup \supp(CA\mathbf{z}) \cup \cdots \cup \supp(CA^{T-1} \mathbf{z}) \rvert > 2q$.
\end{proposition}

Consequently, the following optimal decoder is defined for when the set of attacked nodes is fixed:
\begin{align}
\mathbf{x}_0 = \argmin\limits_{\mathbf{x}} \norm { Y_T - \Phi_T (\mathbf{x}) }_{l_0} 
\end{align}
%where the $l_0$ ``norm" of matrix $M$ is the number of nonzero rows in $M$ \cite{c22}:
%\begin{align}
	%\norm{M} _{l_0} \triangleq \lvert \textsf{rowsupp} (M) \rvert = \lvert \{ i \in \{ 1, ... , m\} | M_i \neq 0 \}  \rvert 
%\end{align}
%where $M_i$ represents the $i$-th row of $M$. 
where
\begin{align*}
Y_T = \left[\begin{array}{c|c|c|c} \mathbf{y}_0 & \mathbf{y}_1 & \hdots &  \mathbf{y}_{T-1} \end{array}\right] \in \mathbb{R}^{m\times T}
\end{align*}
 and $\Phi_T : \mathbb{R}^n\mapsto\mathbb{R}^{m\times T}$ is a linear map given by:
\begin{align*}
\Phi_T (\mathbf{x}) = \left[\begin{array}{c|c|c|c} C\mathbf{x} & CA\mathbf{x}  & \hdots & CA^{T-1} \mathbf{x} \end{array}\right] \in \mathbb{R}^{m\times T}.
\end{align*}

\subsubsection{Secure estimation for Varying Attacked Nodes\cite{hu2016secure}}
Assuming that the set $\mathcal{K}$ of attacked nodes can change with time but bounded as in $\abs{\mathcal{K}}\le q$:
\begin{definition}\label{def:K_variant}
$q$ errors are correctable after $T$ steps by the decoder $\mathcal{D}:\left(\mathbb{R}^m\right)^T\mapsto\mathbb{R}^n$ if for any $\mathbf{x}_0 \in \mathbb{R}^n$ and any sequence of vectors $\mathbf{e}_0,\hdots,\mathbf{e}_{T-1}\in\mathbf{R}^m$ such that $\abs{\textsf{supp}(\mathbf{e}_k)} \leq q$, we have $\mathcal{D}(\mathbf{y}_0,\hdots,\mathbf{y}_{T-1})=\mathbf{x}_0$, where $\mathbf{y}_k = CA^k\mathbf{x}_0 + \mathbf{e}_k$ for $k=0,1,\hdots,T-1$.
\end{definition}

\begin{proposition}
Let $T \in \mathbb{N}  \backslash \{ 0\}$. The following are equivalent:\\
(i) There is a decoder that can correct $q$ errors after $T$ steps;\\
(ii) For all $\mathbf{z}\in \mathbb{R}^n \backslash \{0\}$ , $\sum\limits_{k=0}^{T-1}\abs{\textsf{supp}(CA^k \mathbf{z})} > 2q$.
\end{proposition}

Consequently, the following optimal decoder is defined for when the set of attacked nodes is not fixed:
\begin{align}
\mathbf{x}_0 = \argmin\limits_{\mathbf{x}} \norm { \mathbf{y}_{(T)} - \Phi_{(T)} \mathbf{x} }_{l_0} 
\end{align}
where
\begin{align*}
\mathbf{y}_{(T)} = \left[\begin{array}{c} \mathbf{y}_0\\ \mathbf{y}_1 \\ \vdots \\  \mathbf{y}_{T-1} \end{array}\right] \in \mathbb{R}^{m T},
\end{align*}

\begin{align*}
\Phi_{(T)}  = \left[\begin{array}{c} C\\ CA \\ \vdots \\ CA^{T-1} \end{array}\right] \in \mathbb{R}^{mT \times n}.
\end{align*}
